Clustering Mixtures with Almost Optimal Separation in Polynomial Time

We consider the problem of clustering mixtures of mean-separated Gaussians in high dimensions. We are given samples from a mixture of $k$ identity covariance Gaussians, so that the minimum pairwise distance between any two pairs of means is at least $\Delta$, for some parameter $\Delta > 0$, and the goal is to recover the ground truth clustering of these samples. It is folklore that separation $\Delta = \Theta (\sqrt{\log k})$ is both necessary and sufficient to recover a good clustering, at least information theoretically. However, the estimators which achieve this guarantee are inefficient. We give the first algorithm which runs in polynomial time, and which almost matches this guarantee. More precisely, we give an algorithm which takes polynomially many samples and time, and which can successfully recover a good clustering, so long as the separation is $\Delta = \Omega (\log^{1/2 + c} k)$, for any $c > 0$. Previously, polynomial time algorithms were only known for this problem when the separation was polynomial in $k$, and all algorithms which could tolerate $\textsf{poly}( \log k )$ separation required quasipolynomial time. We also extend our result to mixtures of translations of a distribution which satisfies the Poincar\'{e} inequality, under additional mild assumptions. Our main technical tool, which we believe is of independent interest, is a novel way to implicitly represent and estimate high degree moments of a distribution, which allows us to extract important information about high-degree moments without ever writing down the full moment tensors explicitly.

==> new_attempt.tex <==
\section{New Attempt}


Notation
\begin{itemize}
    \item 
    \[
    M_{2s} = w_1 \flatten( \mu_1^{\otimes s} ) \otimes \flatten( \mu_1^{\otimes s} )  + \dots + 
    \]
\end{itemize}

\begin{algorithm}[H]
\caption{{\sc Iterative Projection Step} }
\begin{algorithmic}
\State \textbf{Input:} Samples $z_1, \dots , z_n$ from unknown mixture
\[
\mcl{M} = w_1 \mcl{D}(\mu_1) + \dots + w_k \mcl{D}(\mu_k)
\]

\State \textbf{Input:}  integer $t > 0$ and threshold $\tau > 0$

\State Set $\Pi_0 = 1$
\State Split samples into $t$ sets $S_1, \dots , S_t$ of equal size
\For{s = 1,2, \dots , t }
\State Run {\sc Estimate Moment Tensor} using samples $S_s$ to get approximation $\wt{A_{2s}} \in \R^{dk \times dk}$ to
\[
A_{2s} = \left(I_d \otimes_\kr \Gamma_{ \Pi_{s-1}, \dots , \Pi_1} \right) M_{2s}\left(I_d \otimes_\kr \Gamma_{ \Pi_{s-1}, \dots , \Pi_1} \right)^T
\]

\State Let $\Pi_s \in \R^{k \times dk}$ have rows forming an orthonormal basis of the top $k$ singular subspace of $\wt{A_{2s}}$
\EndFor
\State \textbf{Output:}  $ (\Pi_t,\dots , \Pi_1)$
\end{algorithmic}
\label{alg:iterative-projection}
\end{algorithm}


\begin{claim}
Assume $\norm{A_{2s}, \wt{A_{2s}}}_F$ can be made smaller than any polynomial.  Then 
\[
\norm{ \Gamma_{ \Pi_{s}, \dots , \Pi_1} \flatten( \mu_i^{s}) } \geq \left( 1 - \frac{1}{\poly} \right) \norm{\mu_i} \norm{ \Gamma_{ \Pi_{s-1}, \dots , \Pi_1} \flatten( \mu_i^{s-1}) }
\]
\end{claim}
\begin{proof}
\[
A_{2s} = \sum w_i \flatten(\mu_i \otimes \Gamma_{ \Pi_{s-1}, \dots , \Pi_1} \flatten( \mu_i^{s-1}))^{\otimes 2}
\]
Let $v$ be the projection of $\mu_i \otimes \Gamma_{ \Pi_{s-1}, \dots , \Pi_1} \flatten( \mu_i^{s-1})$ onto orthogonal complement of $\Pi_s$.  Now I know that
\[
v^T A_{2s} v \geq w_i \norm{v}^4
\]
this is because
\[
\langle v, \mu_i \otimes \Gamma_{ \Pi_{s-1}, \dots , \Pi_1} \flatten( \mu_i^{s-1}) \rangle  = \norm{v}^2
\]
But 
\[
v^T \wt{A_{2s}} v = 0
\]
Also by accuracy assumption
\[
v^T(\wt{A_{2s}} - A_{2s} ) v \leq \eps \norm{v}^2
\]
\end{proof}






\begin{algorithm}[H]
\caption{{\sc Estimate Moment Tensor} }
\begin{algorithmic}
\State \textbf{Input:} Samples $z_1, \dots , z_n$ from unknown mixture
\[
\mcl{M} = w_1 \mcl{D}(\mu_1) + \dots + w_k \mcl{D}(\mu_k)
\]
\State \textbf{Input:} Integer $s > 0$
\State \textbf{Input:} Integers $c_{s-1}, \dots , c_1 \geq 1, c_0 = 1$ and matrices $\Pi_{s-1} \in \R^{c_{s-1} \times dc_{s-2}} \dots \Pi_{1} \in \R^{c_{1} \times dc_0}$ 
\For{i = 1,2, \dots , n}
\State Independently draw samples $x_1, \dots , x_{2s}$ from $\mcl{D}$
\State Compute the $(dc_{s-1})^2$-dimensional vector
\[
X_i = ( (I_d \otimes_{\text{kr}} \Gamma_{\Pi_{s-1}, \dots , \Pi_1}) \otimes_{\text{kr}} (I_d \otimes_{\text{kr}} \Gamma_{\Pi_{s-1}, \dots , \Pi_1})) \flatten \left(Q_{2s}(z_i , x_1, \dots , x_{2s}) \right)
\]

\State Let $K_i$ be the rearrangement of $X_i$ into a square $dc_{s-1} \times dc_{s-1}$-dimensional matrix
\EndFor
\State \textbf{Output:} $A = (K_1 + \dots + K_n)/n$
\end{algorithmic}
\label{alg:est-moment-tensor}
\end{algorithm}



\subsection{Estimating Moments}

Notation
\begin{itemize}
    \item We have some distribution $\mcl{D}$ with mean $0$
    \item We use $T_1, T_2, \dots $ are 
    \[
    T_i = \E_{x \sim \mcl{D}}[ x^{\otimes i}] \,.
    \]
\end{itemize}


There is a unique polynomial such that $\E_{x \sim \mcl{D}(\mu)}[ P_t(x) ] = \mu^{\otimes t}$.  This is given by the following recurrence
\[
P_t(x) = x^{\otimes t} - \sum T_1 \otimes P_{t-1}(x) - \sum T_2 \otimes  P_{t-2}(x) - \dots - T_t
\]

Take derivative w.r.t. $x_1$.  Let $e_1  = (1, \dots , 0)$.  We get
\[
\partial_1 P_t(x) = \sum e_1 \otimes x^{\otimes t-1}  - \sum T_1 \otimes \partial_1 P_{t-1}(x) - \dots - \sum \partial_1 P_1(x) \otimes T_{t-1}
\]
We claim by induction
\[
\partial_i P_{t}(x) = \sum e_i \otimes P_{t-1}(x)
\]
Now we use Poincare to bound
\[
\E_{x \sim \mcl{D}}[  (v \cdot P_t(x) )^2 ] \leq  \E_{x \sim \mcl{D}}[ \sum_{i=1}^d (v \cdot \partial_i P_t(x))^2  ] 
\]
Inductive hypothesis is 
\[
\E_{x \sim \mcl{D}}[  (v \cdot P_t(x) )^2 ] \leq f(t) \norm{v}^2
\]
Then using the previous identity  
\[
\E_{x \sim \mcl{D}}[  (v \cdot \partial_i P_t(x))^2  ]  \leq t \E_{x \sim \mcl{D}}[ \sum_{j = 1}^t\norm{v_{ a_j = i}}^2] 
\]
summing over all $i$
\[
\E_{x \sim \mcl{D}}[  (v \cdot P_t(x) )^2 ] = t^2f(t-1) \norm{v}^2
\]


For non-mean $0$, 
\[
\E_{x \sim \mcl{D}}[  (v \cdot P_t(x) )^2 ] \leq ( \norm{\mu}^2 + t^2)^t \norm{v}^2
\]
The recurrence is 
\[
\E_{x \sim \mcl{D}}[  (v \cdot P_t(x) )^2 ] \leq \norm{\mu}^{2t} \norm{v}^2 + t^2 ( \norm{\mu}^2 + (t-1)^2)^{t-1} \norm{v}^2
\]

